On the stability and performance of the solution of sparse linear systems by partitioned procedures

In this paper, we present, evaluate and analyse the performance of parallel synchronous Jacobi algorithms by different partitioned procedures including band-row splitting, band-row sparsity pattern splitting and substructuring splitting, when solving sparse large linear systems. Numerical experiments performed on a set of academic 3D Laplace equation and on a real gravity matrices arising from the Chicxulub crater are exhibited, and show the impact of splitting on parallel synchronous iterations when solving sparse large linear systems. The numerical results clearly show the interest of substructuring methods compared to band-row splitting strategies.

==> 0_packages/matrix.skeleton/pgflibrarymatrix.skeleton.code.tex <==
\usepgfmodule{matrix}

\def\pgfmatrixlabelskeleton{
  \let\pgf@matrix@compute@origin\pgf@matrix@skeleton@compute@origin
  \let\pgf@matrix@shift@nodes@initial\pgf@matrix@skeleton@shift@nodes@initial
  \let\pgf@end@matrix\pgf@end@matrix@skeleton
}

\expandafter\def\expandafter\pgf@end@matrix@skeleton\expandafter{\pgf@end@matrix \pgf@matrix@create@skeleton}%

% Creates the skeleton

% orig contains the upper left corner of the different boxes

\def\pgf@matrix@create@skeleton{%
  \xdef\pgf@matrix@skel@innerxsep{\pgfkeysvalueof{/pgf/inner xsep}}%
  \xdef\pgf@matrix@skel@innerysep{\pgfkeysvalueof{/pgf/inner ysep}}%
  \pgfscope%
    \pgfgetlastxy\ck@shift@x\ck@shift@y
    \pgftransformshift{\pgfpoint{\ck@shift@x}{\ck@shift@y}}%
    \pgfset{inner sep=0pt}%
    \pgf@matrix@skeleton@create@cells%
    \pgf@matrix@skeleton@create@tiling@cells%
    \pgf@matrix@skeleton@create@rows%
    \pgf@matrix@skeleton@create@tiling@rows%
    \pgf@matrix@skeleton@create@columns%
    \pgf@matrix@skeleton@create@tiling@columns%
  \endpgfscope%
}

\def\pgf@matrix@skeleton@create@cells{%
  \newcount\pgf@matrix@skel@next@row
  \foreach \pgf@matrix@skel@row in {1, ..., \pgfmatrixcurrentrow} {%
    \pgf@matrix@skel@next@row=\pgf@matrix@skel@row
    \advance\pgf@matrix@skel@next@row by 1
    \pgfmathsetmacro{\pgf@matrix@skel@origy}{\csname pgf@matrix@origy\pgf@matrix@skel@row\endcsname + \csname pgf@matrix@maxy\pgf@matrix@skel@row\endcsname}%
    \pgfmathsetmacro{\pgf@matrix@skel@height}{\csname pgf@matrix@maxy\pgf@matrix@skel@row\endcsname - \csname pgf@matrix@miny\pgf@matrix@skel@row\endcsname - \pgflinewidth}%
    \pgfmathsetmacro{\pgf@matrix@skel@height}{\pgf@matrix@skel@height - \csname pgf@matrix@row@sep@\the\pgf@matrix@skel@next@row\endcsname}
    \foreach \pgf@matrix@skel@col in {1, ..., \pgf@matrix@numberofcolumns} {%
      \pgfmathsetmacro{\pgf@matrix@skel@origx}{\csname pgf@matrix@origx\pgf@matrix@skel@col\endcsname + \csname pgf@matrix@minx\pgf@matrix@skel@col\endcsname}%
      \pgfmathsetmacro{\pgf@matrix@skel@width}{\csname pgf@matrix@maxx\pgf@matrix@skel@col\endcsname - \csname pgf@matrix@minx\pgf@matrix@skel@col\endcsname - \pgflinewidth}%
      \ifnum\pgf@matrix@skel@col>1\relax%
        \pgfmathsetmacro{\pgf@matrix@skel@origx}{\pgf@matrix@skel@origx + \csname pgf@matrix@column@sep@\pgf@matrix@skel@col\endcsname}%
        \pgfmathsetmacro{\pgf@matrix@skel@width}{\pgf@matrix@skel@width - \pgflinewidth - \csname pgf@matrix@column@sep@\pgf@matrix@skel@col\endcsname}%
      \fi%
      {%
        \pgfset{minimum width=\pgf@matrix@skel@width, minimum height=\pgf@matrix@skel@height}%
        \pgftransformshift{\pgfpoint{\pgf@matrix@skel@origx pt}{\pgf@matrix@skel@origy pt}}%
        \pgfnode{rectangle}{north west}{}{\pgf@matrix@par@name-cell-\pgf@matrix@skel@row-\pgf@matrix@skel@col}{}%
      }
    }
  }
}

\def\pgf@matrix@skeleton@create@tiling@cells{%
  \newcount\pgf@matrix@skel@next@col
  \newcount\pgf@matrix@skel@next@row
  \foreach \pgf@matrix@skel@row in {1, ..., \pgfmatrixcurrentrow} {%
    \pgf@matrix@skel@next@row=\pgf@matrix@skel@row
    \advance\pgf@matrix@skel@next@row by 1
    \pgfmathsetmacro{\pgf@matrix@skel@origy}{\csname pgf@matrix@origy\pgf@matrix@skel@row\endcsname + \csname pgf@matrix@maxy\pgf@matrix@skel@row\endcsname}%
    \pgfmathsetmacro{\pgf@matrix@skel@height}{\csname pgf@matrix@maxy\pgf@matrix@skel@row\endcsname - \csname pgf@matrix@miny\pgf@matrix@skel@row\endcsname - \pgflinewidth}%
    \ifnum\pgf@matrix@skel@row=1\relax%
      \pgfmathsetmacro{\pgf@matrix@skel@origy}{\pgf@matrix@skel@origy + \pgf@matrix@skel@innerysep}%
      \pgfmathsetmacro{\pgf@matrix@skel@height}{\pgf@matrix@skel@height + \pgf@matrix@skel@innerysep}%
    \fi
    \ifnum\pgf@matrix@skel@row=\pgfmatrixcurrentrow\relax%
      \pgfmathsetmacro{\pgf@matrix@skel@height}{\pgf@matrix@skel@height + \pgf@matrix@skel@innerysep - \pgfmatrixrowsep}%
    \fi
    \ifnum\pgf@matrix@skel@row>1\relax%
      \pgfmathsetmacro{\pgf@matrix@skel@origy}{\pgf@matrix@skel@origy + 0.5 * \csname pgf@matrix@row@sep@\pgf@matrix@skel@row\endcsname}
      \pgfmathsetmacro{\pgf@matrix@skel@height}{\pgf@matrix@skel@height + 0.5 * \csname pgf@matrix@row@sep@\pgf@matrix@skel@row\endcsname}
    \fi
    \ifnum\pgf@matrix@skel@row<\pgfmatrixcurrentrow\relax%
      \pgfmathsetmacro{\pgf@matrix@skel@height}{\pgf@matrix@skel@height - 0.5 * \csname pgf@matrix@row@sep@\the\pgf@matrix@skel@next@row\endcsname}
    \fi
    \foreach \pgf@matrix@skel@col in {1, ..., \pgf@matrix@numberofcolumns} {%
      \pgf@matrix@skel@next@col=\pgf@matrix@skel@col
      \advance\pgf@matrix@skel@next@col by 1
      \pgfmathsetmacro{\pgf@matrix@skel@origx}{\csname pgf@matrix@origx\pgf@matrix@skel@col\endcsname + \csname pgf@matrix@minx\pgf@matrix@skel@col\endcsname}%
      \pgfmathsetmacro{\pgf@matrix@skel@width}{\csname pgf@matrix@maxx\pgf@matrix@skel@col\endcsname - \csname pgf@matrix@minx\pgf@matrix@skel@col\endcsname- \pgflinewidth}%
      \ifnum\pgf@matrix@skel@col=1\relax%
        \pgfmathsetmacro{\pgf@matrix@skel@origx}{\pgf@matrix@skel@origx - \pgf@matrix@skel@innerxsep}%
        \pgfmathsetmacro{\pgf@matrix@skel@width}{\pgf@matrix@skel@width + \pgf@matrix@skel@innerxsep}%
      \fi%
      \ifnum\pgf@matrix@skel@col=\pgf@matrix@numberofcolumns\relax%
        \pgfmathsetmacro{\pgf@matrix@skel@width}{\pgf@matrix@skel@width + \pgf@matrix@skel@innerxsep}%
      \fi%
      \ifnum\pgf@matrix@skel@col<\pgf@matrix@numberofcolumns%
        \pgfmathsetmacro{\pgf@matrix@skel@width}{\pgf@matrix@skel@width + 0.5 * \csname pgf@matrix@column@sep@\the\pgf@matrix@skel@next@col\endcsname}%
      \fi%
      \ifnum\pgf@matrix@skel@col>1%
        \pgfmathsetmacro{\pgf@matrix@skel@origx}{\pgf@matrix@skel@origx + 0.5 * \csname pgf@matrix@column@sep@\pgf@matrix@skel@col\endcsname}%
        \pgfmathsetmacro{\pgf@matrix@skel@width}{\pgf@matrix@skel@width - 0.5 * \csname pgf@matrix@column@sep@\pgf@matrix@skel@col\endcsname}%
      \fi%
      {%
        \pgfset{minimum width=\pgf@matrix@skel@width, minimum height=\pgf@matrix@skel@height}%
        \pgftransformshift{\pgfpoint{\pgf@matrix@skel@origx pt}{\pgf@matrix@skel@origy pt}}%
        \pgfnode{rectangle}{north west}{}{\pgf@matrix@par@name-tiling-cell-\pgf@matrix@skel@row-\pgf@matrix@skel@col}{}%
      }
    }
  }
}

\def\pgf@matrix@skeleton@create@rows{%
  \newcount\pgf@matrix@skel@next@row%
  \pgfmathsetmacro{\pgf@matrix@skel@width}{\csname pgf@matrix@origx\the\pgf@matrix@numberofcolumns\endcsname + \csname pgf@matrix@maxx\the\pgf@matrix@numberofcolumns\endcsname - \pgflinewidth}%
  \pgfmathsetmacro{\pgf@matrix@skel@origx}{\csname pgf@matrix@origx1\endcsname + \csname pgf@matrix@minx1\endcsname}%
  \foreach \pgf@matrix@skel@row in {1, ..., \pgfmatrixcurrentrow} {%
    \pgf@matrix@skel@next@row=\pgf@matrix@skel@row\relax%
    \advance\pgf@matrix@skel@next@row by1\relax%
    \pgfmathsetmacro{\pgf@matrix@skel@origy}{\csname pgf@matrix@origy\pgf@matrix@skel@row\endcsname + \csname pgf@matrix@maxy\pgf@matrix@skel@row\endcsname}%
    \pgfmathsetmacro{\pgf@matrix@skel@height}{\csname pgf@matrix@maxy\pgf@matrix@skel@row\endcsname - \csname pgf@matrix@miny\pgf@matrix@skel@row\endcsname - \csname pgf@matrix@row@sep@\the\pgf@matrix@skel@next@row\endcsname - \pgflinewidth}%
    {%
      \pgfset{minimum width=\pgf@matrix@skel@width, minimum height=\pgf@matrix@skel@height}%
      \pgftransformshift{\pgfpoint{\pgf@matrix@skel@origx pt}{\pgf@matrix@skel@origy pt}}%
      \pgfnode{rectangle}{north west}{}{\pgf@matrix@par@name-row-\pgf@matrix@skel@row}{}%
    }
    \ifnum\pgf@matrix@skel@row<\pgfmatrixcurrentrow\relax%
      \pgfmathsetmacro{\pgf@matrix@skel@origy}{\csname pgf@matrix@origy\the\pgf@matrix@skel@next@row\endcsname + \csname pgf@matrix@maxy\the\pgf@matrix@skel@next@row\endcsname + \csname pgf@matrix@row@sep@\the\pgf@matrix@skel@next@row\endcsname + 0.5 * \pgflinewidth}%
      \pgfmathsetmacro{\pgf@matrix@skel@height}{\csname pgf@matrix@row@sep@\the\pgf@matrix@skel@next@row\endcsname}%
      {%
        \pgfset{minimum width=\pgf@matrix@skel@width, minimum height=\pgf@matrix@skel@height}%
        \pgftransformshift{\pgfpoint{\pgf@matrix@skel@origx pt}{\pgf@matrix@skel@origy pt}}%
        \pgfnode{rectangle}{north west}{}{\pgf@matrix@par@name-inter-row-\pgf@matrix@skel@row}{}%
      }
    \fi%
  }
}

\def\pgf@matrix@skeleton@create@tiling@rows{%
  \newcount\pgf@matrix@skel@next@row%
  \pgfmathsetmacro{\pgf@matrix@skel@width}{\csname pgf@matrix@origx\the\pgf@matrix@numberofcolumns\endcsname + \csname pgf@matrix@maxx\the\pgf@matrix@numberofcolumns\endcsname - \pgflinewidth + 2 * \pgf@matrix@skel@innerxsep}%
  \pgfmathsetmacro{\pgf@matrix@skel@origx}{\csname pgf@matrix@origx1\endcsname + \csname pgf@matrix@minx1\endcsname - \pgf@matrix@skel@innerxsep}%
  \foreach \pgf@matrix@skel@row in {1, ..., \pgfmatrixcurrentrow} {%
    \pgf@matrix@skel@next@row=\pgf@matrix@skel@row\relax%
    \advance\pgf@matrix@skel@next@row by1\relax%
    \pgfmathsetmacro{\pgf@matrix@skel@origy}{\csname pgf@matrix@origy\pgf@matrix@skel@row\endcsname + \csname pgf@matrix@maxy\pgf@matrix@skel@row\endcsname}%
    \pgfmathsetmacro{\pgf@matrix@skel@height}{\csname pgf@matrix@maxy\pgf@matrix@skel@row\endcsname - \csname pgf@matrix@miny\pgf@matrix@skel@row\endcsname - \csname pgf@matrix@row@sep@\the\pgf@matrix@skel@next@row\endcsname - \pgflinewidth}%
    \ifnum\pgf@matrix@skel@row=1\relax%
      \pgfmathsetmacro{\pgf@matrix@skel@origy}{\pgf@matrix@skel@origy + \pgf@matrix@skel@innerysep}%
      \pgfmathsetmacro{\pgf@matrix@skel@height}{\pgf@matrix@skel@height + \pgf@matrix@skel@innerysep}%
    \fi
    \ifnum\pgf@matrix@skel@row=\pgfmatrixcurrentrow\relax%
      \pgfmathsetmacro{\pgf@matrix@skel@height}{\pgf@matrix@skel@height + \pgf@matrix@skel@innerysep}%
    \fi
    \ifnum\pgf@matrix@skel@row>1\relax%
      \pgfmathsetmacro{\pgf@matrix@skel@origy}{\pgf@matrix@skel@origy + 0.5 * \csname pgf@matrix@row@sep@\pgf@matrix@skel@row\endcsname}%
      \pgfmathsetmacro{\pgf@matrix@skel@height}{\pgf@matrix@skel@height + 0.5 * \csname pgf@matrix@row@sep@\pgf@matrix@skel@row\endcsname}%
    \fi%
    \ifnum\pgf@matrix@skel@row<\pgfmatrixcurrentrow\relax%
      \pgfmathsetmacro{\pgf@matrix@skel@height}{\pgf@matrix@skel@height + 0.5 * \csname pgf@matrix@row@sep@\the\pgf@matrix@skel@next@row\endcsname}%
    \fi%
    {%
      \pgfset{minimum width=\pgf@matrix@skel@width, minimum height=\pgf@matrix@skel@height}%
      \pgftransformshift{\pgfpoint{\pgf@matrix@skel@origx pt}{\pgf@matrix@skel@origy pt}}%
      \pgfnode{rectangle}{north west}{}{\pgf@matrix@par@name-tiling-row-\pgf@matrix@skel@row}{}%
    }
  }
}

\def\pgf@matrix@skeleton@create@columns{%
  \newcount\pgf@matrix@skel@prev@col%
  \pgfmathsetmacro{\pgf@matrix@skel@height}{\csname pgf@matrix@origy1\endcsname + \csname pgf@matrix@maxy1\endcsname - \csname pgf@matrix@miny\the\pgfmatrixcurrentrow\endcsname - \pgfmatrixrowsep - \pgflinewidth}%
  \pgfmathsetmacro{\pgf@matrix@skel@origy}{\csname pgf@matrix@origy1\endcsname + \csname pgf@matrix@maxy1\endcsname}%
  \foreach \pgf@matrix@skel@col in {1, ..., \pgf@matrix@numberofcolumns} {%
    \ifnum\pgf@matrix@skel@col>1\relax%
      \pgfmathsetmacro{\pgf@matrix@skel@origx}{\csname pgf@matrix@origx\pgf@matrix@skel@col\endcsname + \csname pgf@matrix@minx\pgf@matrix@skel@col\endcsname + \csname pgf@matrix@column@sep@\pgf@matrix@skel@col\endcsname}%
      \pgfmathsetmacro{\pgf@matrix@skel@width}{\csname pgf@matrix@maxx\pgf@matrix@skel@col\endcsname - \csname pgf@matrix@minx\pgf@matrix@skel@col\endcsname - \csname pgf@matrix@column@sep@\pgf@matrix@skel@col\endcsname - \pgflinewidth}%
    \else%
      \pgfmathsetmacro{\pgf@matrix@skel@origx}{\csname pgf@matrix@origx\pgf@matrix@skel@col\endcsname + \csname pgf@matrix@minx\pgf@matrix@skel@col\endcsname}%
      \pgfmathsetmacro{\pgf@matrix@skel@width}{\csname pgf@matrix@maxx\pgf@matrix@skel@col\endcsname - \csname pgf@matrix@minx\pgf@matrix@skel@col\endcsname - \pgflinewidth}%
    \fi%
    {%
      \pgfset{minimum width=\pgf@matrix@skel@width, minimum height=\pgf@matrix@skel@height}%
      \pgftransformshift{\pgfpoint{\pgf@matrix@skel@origx pt}{\pgf@matrix@skel@origy pt}}%
      \pgfnode{rectangle}{north west}{}{\pgf@matrix@par@name-column-\pgf@matrix@skel@col}{}%
    }
    \ifnum\pgf@matrix@skel@col>1\relax%
      \pgf@matrix@skel@prev@col=\pgf@matrix@skel@col\relax%
      \advance\pgf@matrix@skel@prev@col by-1\relax%
      \pgfmathsetmacro{\pgf@matrix@skel@origx}{\csname pgf@matrix@origx\the\pgf@matrix@skel@prev@col\endcsname + \csname pgf@matrix@maxx\the\pgf@matrix@skel@prev@col\endcsname - 0.5 * \pgflinewidth}%
      \pgfmathsetmacro{\pgf@matrix@skel@width}{\csname pgf@matrix@column@sep@\pgf@matrix@skel@col\endcsname}%
      {%
        \pgfset{minimum width=\pgf@matrix@skel@width, minimum height=\pgf@matrix@skel@height}%
        \pgftransformshift{\pgfpoint{\pgf@matrix@skel@origx pt}{\pgf@matrix@skel@origy pt}}%
        \pgfnode{rectangle}{north west}{}{\pgf@matrix@par@name-inter-column-\the\pgf@matrix@skel@prev@col}{}%
      }
    \fi%
  }
}

\def\pgf@matrix@skeleton@create@tiling@columns{%
  \newcount\pgf@matrix@skel@next@col%
  \pgfmathsetmacro{\pgf@matrix@skel@height}{\csname pgf@matrix@origy1\endcsname + \csname pgf@matrix@maxy1\endcsname - \csname pgf@matrix@miny\the\pgfmatrixcurrentrow\endcsname - \pgfmatrixrowsep - \pgflinewidth + 2 * \pgf@matrix@skel@innerysep}%
  \pgfmathsetmacro{\pgf@matrix@skel@origy}{\csname pgf@matrix@origy1\endcsname + \csname pgf@matrix@maxy1\endcsname + \pgf@matrix@skel@innerysep}%
  \foreach \pgf@matrix@skel@col in {1, ..., \pgf@matrix@numberofcolumns} {%
    \pgf@matrix@skel@next@col=\pgf@matrix@skel@col\relax%
    \advance\pgf@matrix@skel@next@col by1\relax%
    \ifnum\pgf@matrix@skel@col>1\relax%
      \pgfmathsetmacro{\pgf@matrix@skel@origx}{\csname pgf@matrix@origx\pgf@matrix@skel@col\endcsname + \csname pgf@matrix@minx\pgf@matrix@skel@col\endcsname + \csname pgf@matrix@column@sep@\pgf@matrix@skel@col\endcsname}%
      \pgfmathsetmacro{\pgf@matrix@skel@width}{\csname pgf@matrix@maxx\pgf@matrix@skel@col\endcsname - \csname pgf@matrix@minx\pgf@matrix@skel@col\endcsname - \csname pgf@matrix@column@sep@\pgf@matrix@skel@col\endcsname - \pgflinewidth}%
    \else%
      \pgfmathsetmacro{\pgf@matrix@skel@origx}{\csname pgf@matrix@origx\pgf@matrix@skel@col\endcsname + \csname pgf@matrix@minx\pgf@matrix@skel@col\endcsname}%
      \pgfmathsetmacro{\pgf@matrix@skel@width}{\csname pgf@matrix@maxx\pgf@matrix@skel@col\endcsname - \csname pgf@matrix@minx\pgf@matrix@skel@col\endcsname - \pgflinewidth}%
    \fi%
    \ifnum\pgf@matrix@skel@col=1\relax%
      \pgfmathsetmacro{\pgf@matrix@skel@origx}{\pgf@matrix@skel@origx - \pgf@matrix@skel@innerxsep}%
      \pgfmathsetmacro{\pgf@matrix@skel@width}{\pgf@matrix@skel@width + \pgf@matrix@skel@innerxsep}%
    \fi
    \ifnum\pgf@matrix@skel@col=\pgf@matrix@numberofcolumns\relax%
      \pgfmathsetmacro{\pgf@matrix@skel@width}{\pgf@matrix@skel@width + \pgf@matrix@skel@innerxsep}%
    \fi
    \ifnum\pgf@matrix@skel@col>1\relax%
      \pgfmathsetmacro{\pgf@matrix@skel@origx}{\pgf@matrix@skel@origx - 0.5 * \csname pgf@matrix@column@sep@\pgf@matrix@skel@col\endcsname}%
      \pgfmathsetmacro{\pgf@matrix@skel@width}{\pgf@matrix@skel@width + 0.5 * \csname pgf@matrix@column@sep@\pgf@matrix@skel@col\endcsname}%
    \fi
    \ifnum\pgf@matrix@skel@col<\pgf@matrix@numberofcolumns\relax%
      \pgfmathsetmacro{\pgf@matrix@skel@width}{\pgf@matrix@skel@width + 0.5 * \csname pgf@matrix@column@sep@\the\pgf@matrix@skel@next@col\endcsname}%
    \fi
    {%
      \pgfset{minimum width=\pgf@matrix@skel@width, minimum height=\pgf@matrix@skel@height}%
      \pgftransformshift{\pgfpoint{\pgf@matrix@skel@origx pt}{\pgf@matrix@skel@origy pt}}%
      \pgfnode{rectangle}{north west}{}{\pgf@matrix@par@name-tiling-column-\pgf@matrix@skel@col}{}%
    }
  }
}

% Compute the real positions of the origins

% We must now compute the real positions of the origins of all the
% small pictures. To this end, we need to compute prefix sums. After
% the procedure is done, the origx and the origy will contain the origin
% positions.

\def\pgf@matrix@skeleton@compute@origin{%
  %
  % Inverse prefix sum on the vertical positions
  %
  {%
    \ifnum\pgfmatrixcurrentrow>0\relax%
      \expandafter\gdef\csname pgf@matrix@origy\the\pgfmatrixcurrentrow\endcsname{0pt}%
    \fi%
    \c@pgf@counta=\pgfmatrixcurrentrow\relax%
    \loop%
    \ifnum\c@pgf@counta>1\relax%
      \pgf@y=\csname pgf@matrix@origy\the\c@pgf@counta\endcsname\relax%
      \advance\pgf@y by\csname pgf@matrix@maxy\the\c@pgf@counta\endcsname\relax
      \advance\c@pgf@counta by-1\relax%
      \pgf@ya=\csname pgf@matrix@miny\the\c@pgf@counta\endcsname\relax%
      \advance\pgf@y by-\pgf@ya\relax%
      \expandafter\xdef\csname pgf@matrix@origy\the\c@pgf@counta\endcsname{\the\pgf@y}%
    \repeat%
  }%
  %
  % Prefix sum on the horizontal positions
  %
  {%
    \ifnum\pgf@matrix@numberofcolumns>0\relax%
      \pgf@x=\csname pgf@matrix@minx1\endcsname\relax%
      \pgf@x=-\pgf@x%
      \expandafter\xdef\csname pgf@matrix@origx1\endcsname{\the\pgf@x}%
    \fi%
    \c@pgf@counta=1\relax%
    \loop%
    \ifnum\c@pgf@counta<\pgf@matrix@numberofcolumns\relax%
      \pgf@x=\csname pgf@matrix@origx\the\c@pgf@counta\endcsname\relax%
      \advance\pgf@x by\csname pgf@matrix@maxx\the\c@pgf@counta\endcsname\relax%
      \advance\c@pgf@counta by1\relax%
      \pgf@xa=\csname pgf@matrix@minx\the\c@pgf@counta\endcsname\relax%
      \advance\pgf@x by-\pgf@xa\relax%
      \expandafter\xdef\csname pgf@matrix@origx\the\c@pgf@counta\endcsname{\the\pgf@x}%
    \repeat%
  }%
}


% Shift the nodes to their origins

% The following procedure shifts all nodes in
% \pgf@matrix@node@list to their location inside a temporary
% picture. This picture will later be shifted again to its final
% position in the real picture.

\def\pgf@matrix@skeleton@shift@nodes@initial{%
  {%
  \pgfutil@for\pgf@matrix@node@name:=\pgf@matrix@node@list\do{%
    \ifx\pgf@matrix@node@name\pgfutil@empty%
    \else%
      \expandafter\ifx\csname pgf@matrix@node@visited@\pgf@matrix@node@name\endcsname\relax%
        \pgf@shift@node{\pgf@matrix@node@name}{%
          \pgf@x=\csname pgf@matrix@origx%
            \expandafter\expandafter\expandafter\pgfutil@secondoftwo\csname pgf@matrix@node@location@\pgf@matrix@node@name\endcsname\endcsname%
          \pgf@y=\csname pgf@matrix@origy%
            \expandafter\expandafter\expandafter\pgfutil@firstoftwo\csname pgf@matrix@node@location@\pgf@matrix@node@name\endcsname\endcsname%
          }%
        \expandafter\let\csname pgf@matrix@node@visited@\pgf@matrix@node@name\endcsname=\pgfutil@empty%
      \fi%
    \fi%
  }%
  }%
}


% End of line
\def\pgfmatrixendrow{%
  % if the cell contains nothing, the following \let will be at the
  % beginning (macro expansion has stopped here since neither \omit
  % nor \span was found)
  \let\pgf@matrix@signal@cell@end=\pgf@matrix@signal@cell@end%
  &\pgf@matrix@correct@calltrue%
  \global\pgf@matrix@fixedfalse%
  \pgf@y=0pt%
  \pgf@matrix@addtolength\pgf@y{\pgfmatrixrowsep}%
  \pgfutil@ifnextchar[{\pgfmatrixendrow@skip}{
  {
  \advance\pgfmatrixcurrentrow by1\relax % only temporary for the following:
  \expandafter\xdef\csname pgf@matrix@row@sep@\the\pgfmatrixcurrentrow\endcsname{\the\pgf@y}%
  }
  \pgf@matrix@finish@line}%
}

\def\pgfmatrixendrow@skip[#1]{%
  \pgf@matrix@addtolength\pgf@y{#1}%
  {
  \advance\pgfmatrixcurrentrow by1\relax % only temporary for the following:
  \expandafter\xdef\csname pgf@matrix@row@sep@\the\pgfmatrixcurrentrow\endcsname{\the\pgf@y}%
  }
  \pgf@matrix@finish@line%
}


==> 0_packages/matrix.skeleton/tikzlibrarymatrix.skeleton.code.tex <==
%TODO (remove) \usepgflibrary{matrix.skeleton}
%\usepgflibrary{matrix.skeleton}

\usetikzlibrary{matrix}
\usetikzlibrary{fit}
\usetikzlibrary{backgrounds}


\tikzset{
  label skeleton/.code = {
    \pgfmatrixlabelskeleton
  },
  add styling node/.style = {
    append after command = {
      \pgfextra
        \pgfinterruptpath
          % This next line is not useful in CVS. This is protection that was needed in the past for nodes.
          \setbox\tikz@figbox=\box\pgfutil@voidb@x
          #1
        \endpgfinterruptpath
      \endpgfextra
    }
  },
  style odd rows/.style = {
    label skeleton,
    add styling node = {
      \foreach \row in {1, ..., \the\pgfmatrixcurrentrow}{
        \ifodd\row
          \fitandstyle{(\tikzlastnode-row-\row)}{#1}
        \fi
      }
    }
  },
  style even rows/.style = {
    label skeleton,
    add styling node={
      \foreach \row in {1, ..., \the\pgfmatrixcurrentrow}{
        \ifodd\row
        \else
          \fitandstyle{(\tikzlastnode-row-\row)}{#1}
        \fi
      }
    }
  },
  style odd rows on layer/.style 2 args= {
    label skeleton,
    add styling node = {
      \foreach \row in {1, ..., \the\pgfmatrixcurrentrow}{
        \ifodd\row
          \fitandstyle[#1]{(\tikzlastnode-row-\row)}{#2}
        \fi
      }
    }
  },
  style even rows on layer/.style 2 args = {
    label skeleton,
    add styling node={
      \foreach \row in {1, ..., \the\pgfmatrixcurrentrow}{
        \ifodd\row
        \else
          \fitandstyle[#1]{(\tikzlastnode-row-\row)}{#2}
        \fi
      }
    }
  },
  style odd tiling rows/.style = {
    label skeleton,
    add styling node = {
      \foreach \row in {1, ..., \the\pgfmatrixcurrentrow}{
        \ifodd\row
          \fitandstyle{(\tikzlastnode-tiling-row-\row)}{#1}
        \fi
      }
    }
  },
  style even tiling rows/.style = {
    label skeleton,
    add styling node={
      \foreach \row in {1, ..., \the\pgfmatrixcurrentrow}{
        \ifodd\row
        \else
          \fitandstyle{(\tikzlastnode-tiling-row-\row)}{#1}
        \fi
      }
    }
  },
  style odd tiling rows on layer/.style 2 args= {
    label skeleton,
    add styling node = {
      \foreach \row in {1, ..., \the\pgfmatrixcurrentrow}{
        \ifodd\row
          \fitandstyle[#1]{(\tikzlastnode-tiling-row-\row)}{#2}
        \fi
      }
    }
  },
  style even tiling rows on layer/.style 2 args = {
    label skeleton,
    add styling node={
      \foreach \row in {1, ..., \the\pgfmatrixcurrentrow}{
        \ifodd\row
        \else
          \fitandstyle[#1]{(\tikzlastnode-tiling-row-\row)}{#2}
        \fi
      }
    }
  },
  style odd columns/.style = {
    label skeleton,
    add styling node = {
      \foreach \col in {1, ..., \the\pgf@matrix@numberofcolumns}{
        \ifodd\col
          \fitandstyle{(\tikzlastnode-column-\col)}{#1}
        \fi
      }
    }
  },
  style even columns/.style = {
    label skeleton,
    add styling node={
      \foreach \col in {1, ..., \the\pgf@matrix@numberofcolumns}{
        \ifodd\col
        \else
          \fitandstyle{(\tikzlastnode-column-\col)}{#1}
        \fi
      }
    }
  },
  style odd columns on layer/.style 2 args= {
    label skeleton,
    add styling node = {
      \foreach \col in {1, ..., \the\pgf@matrix@numberofcolumns}{
        \ifodd\col
          \fitandstyle[#1]{(\tikzlastnode-column-\col)}{#2}
        \fi
      }
    }
  },
  style even columns on layer/.style 2 args = {
    label skeleton,
    add styling node={
      \foreach \col in {1, ..., \the\pgf@matrix@numberofcolumns}{
        \ifodd\col
        \else
          \fitandstyle[#1]{(\tikzlastnode-column-\col)}{#2}
        \fi
      }
    }
  },
  style odd tiling columns/.style = {
    label skeleton,
    add styling node = {
      \foreach \col in {1, ..., \the\pgf@matrix@numberofcolumns}{
        \ifodd\col
          \fitandstyle{(\tikzlastnode-tiling-column-\col)}{#1}
        \fi
      }
    }
  },
  style even tiling columns/.style = {
    label skeleton,
    add styling node={
      \foreach \col in {1, ..., \the\pgf@matrix@numberofcolumns}{
        \ifodd\col
        \else
          \fitandstyle{(\tikzlastnode-tiling-column-\col)}{#1}
        \fi
      }
    }
  },
  style odd tiling columns on layer/.style 2 args= {
    label skeleton,
    add styling node = {
      \foreach \col in {1, ..., \the\pgf@matrix@numberofcolumns}{
        \ifodd\col
          \fitandstyle[#1]{(\tikzlastnode-tiling-column-\col)}{#2}
        \fi
      }
    }
  },
  style even tiling columns on layer/.style 2 args = {
    label skeleton,
    add styling node={
      \foreach \col in {1, ..., \the\pgf@matrix@numberofcolumns}{
        \ifodd\col
        \else
          \fitandstyle[#1]{(\tikzlastnode-tiling-column-\col)}{#2}
        \fi
      }
    }
  },
  style contour/.style = {%
    label skeleton,
    add styling node = {
      \stylecontour{#1}
    }
  },
  style contour on layer/.style 2 args= {%
    label skeleton,
    add styling node = {
      \pgfonlayer{#1}
        \stylecontour{#2}
      \endpgfonlayer
    }
  },
  style grid/.style = {%
    label skeleton,
    add styling node = {
      \stylegrid{#1}
    }
  },
  style grid on layer/.style 2 args= {%
    label skeleton,
    add styling node = {
      \pgfonlayer{#1}
        \stylegrid{#2}
      \endpgfonlayer
    }
  },
  style tiling grid/.style = {%
    label skeleton,
    add styling node = {
      \styletilinggrid{#1}
    }
  },
  style tiling grid on layer/.style 2 args= {%
    label skeleton,
    add styling node = {
      \pgfonlayer{#1}
        \styletilinggrid{#2}
      \endpgfonlayer
    }
  },
}

\def\fitandstyle{\@ifnextchar[{\fitandstyle@layer}{\fitandstyle@main}}
\def\fitandstyle@layer[#1]#2#3{
  \pgfonlayer{#1}
    \fitandstyle@main{#2}{#3}
  \endpgfonlayer
}
\def\fitandstyle@main#1#2{\node [fit = #1, inner sep = 0pt, #2] {};}

\def\stylecontour#1{
  \path [#1] (\tikzlastnode-row-1.north west) -- (\tikzlastnode-row-1.north east) -- (\tikzlastnode-row-\the\pgfmatrixcurrentrow.south east) -- (\tikzlastnode-row-\the\pgfmatrixcurrentrow.south west) -- cycle;
}

\def\stylegrid#1{
  \ifnum\the\pgfmatrixcurrentrow>1\relax%
    \foreach \row in {1, ..., \the\pgfmatrixcurrentrow}{
      \ifnum\row<\the\pgfmatrixcurrentrow\relax%
        \path [#1] (\tikzlastnode-inter-row-\row.west) -- (\tikzlastnode-inter-row-\row.east);
      \fi
    }
  \fi
  \ifnum\the\pgf@matrix@numberofcolumns>1\relax%
    \foreach \column in {1, ..., \the\pgf@matrix@numberofcolumns}{
      \ifnum\column<\the\pgf@matrix@numberofcolumns\relax%
        \path [#1] (\tikzlastnode-inter-column-\column.north) -- (\tikzlastnode-inter-column-\column.south);
      \fi
    }
  \fi
}

\def\styletilinggrid#1{
  \ifnum\the\pgfmatrixcurrentrow>1\relax%
    \foreach \row in {1, ..., \the\pgfmatrixcurrentrow}{
      \ifnum\row<\the\pgfmatrixcurrentrow\relax%
        \path [#1] (\tikzlastnode-tiling-row-\row.south west) -- (\tikzlastnode-tiling-row-\row.south east);
      \fi
    }
  \fi
  \ifnum\the\pgf@matrix@numberofcolumns>1\relax%
    \foreach \column in {1, ..., \the\pgf@matrix@numberofcolumns}{
      \ifnum\column<\the\pgf@matrix@numberofcolumns\relax%
        \path [#1] (\tikzlastnode-tiling-column-\column.north east) -- (\tikzlastnode-tiling-column-\column.south east);
      \fi
    }
  \fi
}


==> 0_packages/pgfornament/am/pgflibraryam.code.tex <==
% utf8
% author Alain Matthes d'après des travaux de F Fradin et H Voss  sur un fichier
% 21/01/2012
\makeatletter

% dimensions des motifs
\def\@pgfornamentDim#1{% dim en bp
\ifcase#1\relax%
\or\def\@pgfornamentX{136}\def\@pgfornamentY{107}% 1
\or\def\@pgfornamentX{133}\def\@pgfornamentY{48}%  2
\fi%
}%
% appels des motifs 
\def\pgf@@ornament#1{%
\begingroup
\def\i{\pgfusepath{clip}}
\let\o\pgfpathclose
\let\s\pgfusepathqfillstroke
\def\p ##1##2{\pgfqpoint{##1bp}{##2bp}}
\def\m ##1 ##2 {\pgfpathmoveto{\p{##1}{##2}}}
\def\l ##1 ##2 {\pgfpathlineto{\p{##1}{##2}}}
\def\r ##1 ##2 ##3 ##4 {\pgfpathrectangle{\p{##1}{##2}}{\p{##3}{##4}}}
\def\c ##1 ##2 ##3 ##4 ##5 ##6 {%
\pgfpathcurveto{\p{##1}{##2}}{\p{##3}{##4}}{\p{##5}{##6}}}%
\@@input am#1.pgf 
%\@nameuse{pgf@@am@#1}%
\endgroup}%
\makeatother
\endinput   

==> 0_packages/pgfornament/vectorian/pgflibraryvectorian.code.tex <==
% utf8
% author Alain Matthes d'après des travaux de F Fradin et H Voss  sur un fichier
% 21/01/2012
\makeatletter
% dimensions des motifs
\def\@pgfornamentDim#1{% dim en bp
\ifcase#1\relax%
\or\def\@pgfornamentX{136}\def\@pgfornamentY{107}% 1
\or\def\@pgfornamentX{134}\def\@pgfornamentY{48}%  2
\or\def\@pgfornamentX{130}\def\@pgfornamentY{65}%  3
\or\def\@pgfornamentX{133}\def\@pgfornamentY{133}% 4
\or\def\@pgfornamentX{129}\def\@pgfornamentY{146}% 5
\or\def\@pgfornamentX{134}\def\@pgfornamentY{148}% 6
\or\def\@pgfornamentX{136}\def\@pgfornamentY{135}% 7
\or\def\@pgfornamentX{134}\def\@pgfornamentY{134}% 8
\or\def\@pgfornamentX{79}\def\@pgfornamentY{105}% 9
\or\def\@pgfornamentX{80}\def\@pgfornamentY{99}%  10
\or\def\@pgfornamentX{123}\def\@pgfornamentY{67}%  11
\or\def\@pgfornamentX{136}\def\@pgfornamentY{136}% 12
\or\def\@pgfornamentX{136}\def\@pgfornamentY{236}% 13
\or\def\@pgfornamentX{123}\def\@pgfornamentY{67}%  14
\or\def\@pgfornamentX{103}\def\@pgfornamentY{52}%  15
\or\def\@pgfornamentX{103}\def\@pgfornamentY{52}%  16
\or\def\@pgfornamentX{74}\def\@pgfornamentY{59}%  17
\or\def\@pgfornamentX{74}\def\@pgfornamentY{59}%  18
\or\def\@pgfornamentX{81}\def\@pgfornamentY{81}%  19
\or\def\@pgfornamentX{81}\def\@pgfornamentY{81}%  20
\or\def\@pgfornamentX{70}\def\@pgfornamentY{58}%  21
\or\def\@pgfornamentX{34}\def\@pgfornamentY{61}%  22
\or\def\@pgfornamentX{68}\def\@pgfornamentY{55}%  23
\or\def\@pgfornamentX{79}\def\@pgfornamentY{76}%  24
\or\def\@pgfornamentX{80}\def\@pgfornamentY{88}%  25
\or\def\@pgfornamentX{59}\def\@pgfornamentY{120}% 26
\or\def\@pgfornamentX{101}\def\@pgfornamentY{98}%  27
\or\def\@pgfornamentX{52}\def\@pgfornamentY{102}% 28
\or\def\@pgfornamentX{65}\def\@pgfornamentY{65}%  29
\or\def\@pgfornamentX{63}\def\@pgfornamentY{64}%  30
\or\def\@pgfornamentX{48}\def\@pgfornamentY{48}%  31
\or\def\@pgfornamentX{48}\def\@pgfornamentY{48}%  32
\or\def\@pgfornamentX{85}\def\@pgfornamentY{85}%  33
\or\def\@pgfornamentX{85}\def\@pgfornamentY{85}%  34
\or\def\@pgfornamentX{97}\def\@pgfornamentY{97}%  35
\or\def\@pgfornamentX{97}\def\@pgfornamentY{97}%  36
\or\def\@pgfornamentX{105}\def\@pgfornamentY{104}% 37
\or\def\@pgfornamentX{105}\def\@pgfornamentY{104}% 38
\or\def\@pgfornamentX{112}\def\@pgfornamentY{112}% 39
\or\def\@pgfornamentX{112}\def\@pgfornamentY{112}% 40
\or\def\@pgfornamentX{111}\def\@pgfornamentY{113}% 41
\or\def\@pgfornamentX{111}\def\@pgfornamentY{113}% 42
\or\def\@pgfornamentX{123}\def\@pgfornamentY{63}%  43
\or\def\@pgfornamentX{123}\def\@pgfornamentY{63}%  44
\or\def\@pgfornamentX{385}\def\@pgfornamentY{64}%  45
\or\def\@pgfornamentX{453}\def\@pgfornamentY{97}%  46
\or\def\@pgfornamentX{114}\def\@pgfornamentY{32}%  47
\or\def\@pgfornamentX{114}\def\@pgfornamentY{32}%  48
\or\def\@pgfornamentX{163}\def\@pgfornamentY{61}%  49
\or\def\@pgfornamentX{164}\def\@pgfornamentY{125}% 50
\or\def\@pgfornamentX{164}\def\@pgfornamentY{125}% 51
\or\def\@pgfornamentX{248}\def\@pgfornamentY{197}% 52
\or\def\@pgfornamentX{134}\def\@pgfornamentY{134}% 53
\or\def\@pgfornamentX{134}\def\@pgfornamentY{134}% 54
\or\def\@pgfornamentX{269}\def\@pgfornamentY{116}% 55
\or\def\@pgfornamentX{269}\def\@pgfornamentY{116}% 56
\or\def\@pgfornamentX{207}\def\@pgfornamentY{103}% 57
\or\def\@pgfornamentX{228}\def\@pgfornamentY{116}% 58
\or\def\@pgfornamentX{204}\def\@pgfornamentY{102}% 59
\or\def\@pgfornamentX{451}\def\@pgfornamentY{189}% 60
\or\def\@pgfornamentX{205}\def\@pgfornamentY{205}% 61
\or\def\@pgfornamentX{205}\def\@pgfornamentY{205}% 62
\or\def\@pgfornamentX{212}\def\@pgfornamentY{212}% 63
\or\def\@pgfornamentX{212}\def\@pgfornamentY{212}% 64
\or\def\@pgfornamentX{132}\def\@pgfornamentY{166}% 65
\or\def\@pgfornamentX{177}\def\@pgfornamentY{175}% 66
\or\def\@pgfornamentX{80}\def\@pgfornamentY{155}% 67
\or\def\@pgfornamentX{361}\def\@pgfornamentY{154}% 68
\or\def\@pgfornamentX{448}\def\@pgfornamentY{227}% 69
\or\def\@pgfornamentX{226}\def\@pgfornamentY{79}%  70
\or\def\@pgfornamentX{443}\def\@pgfornamentY{81}%  71
\or\def\@pgfornamentX{216}\def\@pgfornamentY{58}%  72
\or\def\@pgfornamentX{216}\def\@pgfornamentY{58}%  73
\or\def\@pgfornamentX{308}\def\@pgfornamentY{93}%  74
\or\def\@pgfornamentX{373}\def\@pgfornamentY{120}% 75
\or\def\@pgfornamentX{308}\def\@pgfornamentY{93}%  76
\or\def\@pgfornamentX{207}\def\@pgfornamentY{89}%  77
\or\def\@pgfornamentX{207}\def\@pgfornamentY{132}% 78
\or\def\@pgfornamentX{249}\def\@pgfornamentY{122}% 79
\or\def\@pgfornamentX{454}\def\@pgfornamentY{31}%  80
\or\def\@pgfornamentX{176}\def\@pgfornamentY{45}%  81
\or\def\@pgfornamentX{454}\def\@pgfornamentY{24}%  82
\or\def\@pgfornamentX{449}\def\@pgfornamentY{20}%  83
\or\def\@pgfornamentX{290}\def\@pgfornamentY{57}%  84
\or\def\@pgfornamentX{453}\def\@pgfornamentY{22}%  85
\or\def\@pgfornamentX{454}\def\@pgfornamentY{17}%  86
\or\def\@pgfornamentX{360}\def\@pgfornamentY{44}%  87
\or\def\@pgfornamentX{454}\def\@pgfornamentY{15}%  88
\or\def\@pgfornamentX{454}\def\@pgfornamentY{10}%  89
\fi%
}%
\makeatother
\endinput
